LADs: Leveraging LLMs for AI-Driven DevOps

Automating cloud configuration and deployment remains a critical challenge due to evolving infrastructures, heterogeneous hardware, and fluctuating workloads. Existing solutions lack adaptability and require extensive manual tuning, leading to inefficiencies and misconfigurations. We introduce LADs, the first LLM-driven framework designed to tackle these challenges by ensuring robustness, adaptability, and efficiency in automated cloud management. Instead of merely applying existing techniques, LADs provides a principled approach to configuration optimization through in-depth analysis of what optimization works under which conditions. By leveraging Retrieval-Augmented Generation, Few-Shot Learning, Chain-of-Thought, and Feedback-Based Prompt Chaining, LADs generates accurate configurations and learns from deployment failures to iteratively refine system settings. Our findings reveal key insights into the trade-offs between performance, cost, and scalability, helping practitioners determine the right strategies for different deployment scenarios. For instance, we demonstrate how prompt chaining-based adaptive feedback loops enhance fault tolerance in multi-tenant environments and how structured log analysis with example shots improves configuration accuracy. Through extensive evaluations, LADs reduces manual effort, optimizes resource utilization, and improves system reliability. By open-sourcing LADs, we aim to drive further innovation in AI-powered DevOps automation.

==> Motivation.tex <==
\section{Motivation}
\label{sec:Motivation}

The configuration, deployment, and maintenance of cloud applications demand extensive expertise and a comprehensive understanding of application behaviors across various conditions. Despite technological advancements, these tasks remain complex, primarily due to the dynamic nature of cloud environments and the sensitivity of applications to system specifications and resource allocations.

Modern software systems at leading tech companies like Meta and Google undertake hundreds to thousands of configuration changes on a daily basis. At Meta, for example, thousands of configuration file "diffs" are committed daily, outpacing the frequency of code changes~\cite{lian2024configuration}. This high velocity of configuration changes inevitably leads to misconfigurations, which are among the dominating causes of production incidents. Such statistics underscore the challenges and critical need for efficient configuration management systems that can handle the scale and complexity of modern cloud applications.

Recent studies show that $77\%$ of organizations depend on DevOps to deploy their services, yet many struggle with effective implementation. This struggle is primarily due to the significant amount of time required for various DevOps tasks. For instance, DevOps teams are responsible for $54\%$ of the time in activities related to observability, monitoring, and security, which are crucial for maintaining system stability and performance~\cite{cloudzero2024devops}. However, only 3 in 10 organizations have a clear understanding of their cloud spend, highlighting a gap in the effective management of resources and budgeting in cloud environments. This lack of visibility can lead to inefficient resource usage and increased costs, further complicating the tasks of DevOps teams~\cite{cloudzero2024devops}.

Current methodologies struggle with the significant amount of time DevOps engineers must invest in various critical tasks. The study by Lian et al. on configuration validation reveals that despite extensive efforts to include configuration validators in mature projects, many parameters remain uncovered, highlighting the insufficiency of existing practices. These efforts are known to be costly and often incomprehensive, with a large-scale system exposing hundreds to thousands of configuration parameters, making it challenging to implement validators for every parameter.

The LADS system is proposed to mitigate these challenges by leveraging Large Language Models (LLMs) to automate and optimize the configuration and maintenance processes. By integrating advanced machine learning techniques and contemporary AI research, LADS introduces a novel approach that not only predicts optimal configurations but also automates routine maintenance tasks. This system aims to reduce the cognitive load on developers and enhance the overall efficiency of cloud application management, thereby aligning technical capabilities with business needs more effectively.



==> tables/Pgsql_Table.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{c|lccccccccc}
\noalign{\hrule height 1pt} 
\multirow{2}{*}{\footnotesize \textbf{\begin{tabular}[c]{@{}c@{}}Language\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\footnotesize\textbf{Optimizations}}} & \multicolumn{6}{c|}{\footnotesize\textit{\textbf{Levels}}} & \multirow{2}{*}{\footnotesize \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Accuracy\end{tabular}}} \\ \cline{3-8} 
 & \multicolumn{1}{c|}{} & \footnotesize\textbf{1 $(\uparrow)$} & \multicolumn{1}{c}{\footnotesize\textbf{2 $(\uparrow)$}} & \footnotesize\textbf{3 $(\uparrow)$} & \multicolumn{1}{c}{\footnotesize\textbf{4 $(\uparrow)$}} & \footnotesize\textbf{5 $(\uparrow)$} & \multicolumn{1}{c|}{\footnotesize\textbf{6 $(\uparrow)$}} \\

% \hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{CodeLlama 7b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} &  & &  & &  & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 0 & 0 & 0 & 0 & 0 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 10 & 0 & 20 & 0 & 10 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 40 & 0 & 100 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{LADs}} & \cellcolor{pink!50}40 & \cellcolor{pink!50}30 & \cellcolor{pink!50}100 & \cellcolor{pink!50}0 & \cellcolor{pink!50}30 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \textbf{}\\
% \hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{CodeLlama 13b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 10 & 0 & 10 & 0 & 10 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 10 & 0 & 10 & 0 & 0 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 20 & 10 & 10 & 0 & 10 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 60 & 90 & 90 & 0 & 20 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{LADs}} & \cellcolor{pink!50}90 & \cellcolor{pink!50}80 & \cellcolor{pink!50}80 & \cellcolor{pink!50}10 & \cellcolor{pink!50}30 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \textbf{}\\
% \hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{Llama 3.1 8b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 30 & 0 & 40 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 0 & 0 & 30 & 0 & 20 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 40 & 0 & 40 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 100 & 60 & 100 & 10 & 60 & \multicolumn{1}{l|}{0} & \textbf{}\\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{LADs}} & \cellcolor{pink!50}90 & \cellcolor{pink!50}30 & \cellcolor{pink!50}100 & \cellcolor{pink!50}30 & \cellcolor{pink!50}50 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \\
% \hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{DeepSeekV2 16b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 10 & 0 & 10 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 20 & 30 & 30 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 10 & 10 & 20 & 0 & 20 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 80 & 80 & 90 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{LADs}} & \cellcolor{pink!50}80 & \cellcolor{pink!50}80 & \cellcolor{pink!50}100 & \cellcolor{pink!50}0 & \cellcolor{pink!50}40 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \textbf{}\\
% \hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{Qwen2.5 7b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 30 & 30 & 30 & 0 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 40 & 0 & 30 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 20 & 30 & 10 & 0 & 30 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 90 & 90 & 100 & 0 & 50 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{LADs}} & \cellcolor{pink!50}100 & \cellcolor{pink!50}90 & \cellcolor{pink!50}100 & \cellcolor{pink!50}0 & \cellcolor{pink!50}50 & \multicolumn{1}{l|}{\cellcolor{pink!50}0} & \textbf{}\\
% \hline
\hline

\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{{Qwen2.5 14b}}\end{tabular}}
 & \multicolumn{1}{l|}{\textbf{Vanilla}} & 90 & 60 & 90 & 10 & 40 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{CoT}} & 80 & 50 & 70 & 20 & 50 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\textbf{RAG}} & 20 & 30 & 10 & 0 & 30 & \multicolumn{1}{l|}{20} & \\
 & \multicolumn{1}{l|}{\textbf{FSL}} & 100 & 90 & 100 & 0 & 50 & \multicolumn{1}{l|}{0} & \\
 & \multicolumn{1}{l|}{\cellcolor{pink!50}\textbf{LADs}} & \cellcolor{pink!50}100 & \cellcolor{pink!50}90 & \cellcolor{pink!50}100 & \cellcolor{pink!50}40 & \cellcolor{pink!50}50 & \multicolumn{1}{l|}{\cellcolor{pink!50}30} & \textbf{\underline{}}\\

% \hline

\noalign{\hrule height 1pt}
\end{tabular}
\caption{\textbf{Performance of Various LLMs on PostgreSQL Application with Different Language Models and Optimizations.}
This table presents the accuracy of different large language models (LLMs) on a PostgreSQL application under various optimization strategies across multiple difficulty levels. The optimizations include Vanilla (no optimization), CoT, RAG, FSL, and LADs. The highest-performing optimization for each LLM is highlighted in bold, while the overall best-performing LLM-optimization pair is highlighted in bold and underlined.}
\label{table:PostgreSQL_Table}
\end{table*}
